Quadboost: A Scalable Concurrent Quadtree

Building concurrent spatial trees is more complicated than binary search trees since a space hierarchy should be preserved during modifications. We present a non-blocking quadtree-quadboost-that supports concurrent insert, remove, move, and contain operations. To increase its concurrency, we propose a decoupling approach that separates physical adjustment from logical removal within the remove operation. In addition, we design a continuous find mechanism to reduce its search cost. The move operation combines the searches for different keys together and modifies different positions with atomicity. The experimental results show that quadboost scales well on a multi-core system with 32 hardware threads. More than that, it outperforms existing concurrent trees in retrieving two-dimensional keys with up to 109% improvement when the number of threads is large. The move operation proved to perform better than the best-known algorithm, with up to 47%.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> help <==
obs
\label{obs: leaf key}
The key field of a \textit{Leaf} node is never changed.
\label{obs: space info}
The space information--$\langle x, y, w, h\rangle$ of an \textit{Internal} node is never changed.
\label{obs: root}
The root node is never changed.
\label{obs: two layers}
The tree is initialized with two layers of \textit{Internal} nodes.

defi
\label{defi: find conditions}
The pre-conditions of find(l, pOp, path, keyX, keyY) invoked at $T_{i}$:
\label{defi: findCommon}
The pre-conditions of findCommon(il, rl, lca, rOp, iOp, iPath, rPath, oldKeyX, oldKeyY, newKeyX, newKeyY) invoked at $T_{i}$:


cor
\label{cor: common path}
Two nodes in the quadtree must share a common search path that contains at least two nodes starting from the root.

\label{cor: help pOp}

\label{cor: flag before replace}
A successful $replace$ which belongs to an $op$ will not succeed before it's $flag$ operations have been done.

lem
\label{lem: find first}
At the first time calling the find function, the contain operation, the insert operation, and the remove function start with $l$ as an \textit{Internal} node. 

\label{lem: findCommon first}
At the first time the move operation calls the findCommon function, it starts with \textit{rl} as an \textit{Internal} node. 

\label{lem: find continueFind push nodes}
All nodes pushed by the find function (line~\ref{quadboost: find}) and the continueFind function (line~\ref{quadboost: continueFind}) are \textit{Internal} nodes.

\label{lem: continueFind continueFindCommon push nodes}
All nodes pushed by the findCommon function (line~\ref{quadboost: findCommon}) the continueFindCommon function (line~\ref{quadboost: continueFindCommon}) are \textit{Internal}.

\label{lem: find findCommon process}
For the loop in the find function at line~\ref{quadboost: find} and the findCommon function at line~\ref{quadboost: findCommon}, we suppose that $path$($rPath$) is empty and refer $l$($rl$) and $pOp$($rOp$) to each field updated by the loop. If the loop executes at least once and breaks at $T_{i}$, $l$($rl$), $pOp$($rOp$), and $path$($rPath$) satisfy following conditions:

\label{lem: find pre-condition post-conditions}
Every call to the find function satisfies its pre-condition and post-conditions.

\label{lem: findCommon pre-condition post-conditions}
Every call the findCommon function satisfies its pre-conditions and post-conditions.

\label{lem: continueFind pre-condition post-conditions}
Every call to the continueFind function satisfies its pre-condition and post-conditions.

\label{lem: continueFindCommon pre-conditions post-conditions}

\label{lem: compress pre-conditions}

\label{lem: check pre-conditions}
Every call to the check function satisfies its pre-conditions that $p$ is an \textit{Internal} node.

\label{lem: same type}

\label{lem: helpFlag}

\label{lem: createNode pre-conditions and post-condition}

\label{lem: helpReplace}

\label{lem: op properties}

\label{lem: helpReplace oldChild}
For $helpReplace(p, oldChild, newChild)$ invoked at $T_{i}$, $p$ is an $Internal$ node that has contained $oldChild$ at $T_{i1} < T_{i}$.

